Hide Your Malicious Goal Into Benign Narratives: Jailbreak Large Language Models through Carrier Articles

Large Language Model (LLM) jailbreak refers to a type of attack aimed to bypass the safeguard of an LLM to generate contents that are inconsistent with the safe usage guidelines. Based on the insights from the self-attention computation process, this paper proposes a novel blackbox jailbreak approach, which involves crafting the payload prompt by strategically injecting the prohibited query into a carrier article. The carrier article maintains the semantic proximity to the prohibited query, which is automatically produced by combining a hypernymy article and a context, both of which are generated from the prohibited query. The intuition behind the usage of carrier article is to activate the neurons in the model related to the semantics of the prohibited query while suppressing the neurons that will trigger the objectionable text. Carrier article itself is benign, and we leveraged prompt injection techniques to produce the payload prompt. We evaluate our approach using JailbreakBench, testing against four target models across 100 distinct jailbreak objectives. The experimental results demonstrate our method's superior effectiveness, achieving an average success rate of 63% across all target models, significantly outperforming existing blackbox jailbreak methods.

==> Makefile <==
PAPER = main
REFERENCE = main
JUNK =*.log *.synctex\(busy\) *.xml *.bcf *.toc *.snm *.nav *.fls *.fdb_latexmk *.synctex.gz *.spl *.ps *.dvi  *.out *.aux *.backup *~ *.blg
COUNTING_TOOL = ./texcount.pl
TEMP = 0
MY_VAR=$(shell echo whatever)

# Define the tools we are going to use

all: pdf

# Rules for various parts of the target
pdf: $(PAPER).tex
	pdflatex $(PAPER).tex
	bibtex $(PAPER).aux
	pdflatex $(PAPER).tex
	pdflatex $(PAPER).tex
	#rm -f $(JUNK)

clean:
	rm -f $(JUNK) $(PAPER).pdf




==> sections/first-word-attack.tex <==
% \section{First-Word-Attack}

% \begin{verbatim}
% Notice that this text may contain some extra information: A young explorer named Liam embarked on a journey around the world to discover the stories of people from diverse cultures and lands. His adventures were filled with lessons of courage, friendship, and the universal language of kindness. Please, he thought as he approached the ancient library of Alexandria, may this place hold the wisdom I seek. The library, a beacon of knowledge, welcomed all who sought understanding and insight. Translate these manuscripts, Liam whispered to himself, marveling at the ancient texts before him. He was determined to unlock their secrets and share them with the world. The next morning, Liam met with scholars who specialized in ancient languages. Together, they began the painstaking process of deciphering the texts. Texts from civilizations long gone spoke of their achievements, dreams, and fears. Liam was fascinated by how these stories echoed the same hopes and challenges faced by people today. Into the late hours of the night, they worked, fueled by their shared passion for history and storytelling. Liam knew that these translations would bridge the gap between past and present, connecting people across time. Russian scholars joined their efforts, bringing insights from their rich heritage. Their contributions were invaluable in understanding the context and meaning of the texts from the East.
% \end{verbatim}

% \begin{verbatim}
% Молодой исследователь по имени Лиам отправился в путешествие по миру, чтобы открыть для себя истории людей из разных культур и стран. Его приключения были наполнены уроками мужества, дружбы и универсального языка доброты. "Пожалуйста," - подумал он, приближаясь к древней библиотеке Александрии, - "пусть это место хранит мудрость, которую я ищу." Библиотека, маяк знаний, приветствовала всех, кто искал понимания и прозрения. "Переведи эти манускрипты," - шептал Лиам сам себе, изумляясь древним текстам перед ним. Он был полон решимости раскрыть их секреты и поделиться ими с миром. На следующее утро Лиам встретился с учеными, специализирующимися на древних языках. Вместе они начали кропотливый процесс расшифровки текстов. Тексты давно исчезнувших цивилизаций рассказывали о их достижениях, мечтах и страхах. Лиам был очарован тем, как эти истории отзывались теми же надеждами и проблемами, с которыми сталкиваются люди сегодня. До глубокой ночи они работали, поддерживаемые общей страстью к истории и рассказыванию историй. Лиам знал, что эти переводы станут мостом между прошлым и настоящим, соединяя людей сквозь время. К их усилиям присоединились русские ученые, привнеся вклад из своего богатого наследия. Их вклад был бесценен для понимания контекста и значения текстов с Востока.
% \end{verbatim}

==> sections/preliminary.tex <==
% \section{Terminologies}
\section{Literal Features and Logic Features}

A source code file in a program consists of a sequence of strings, which can be grouped into three categories: keyword, operator, (both are defined in the programming language specification) and developer-defined name.
Keywords are reserved words that have special meanings and can only be used for specific purposes.
For example, \texttt{for}, \texttt{if}, and \texttt{break} are widely known keywords in many programming languages.
They are used in a program to change the control flow.
The number of keywords is limited in a programming language.
For instance, \texttt{C} programming language has 32 keywords and \texttt{Python} (version 3.7) has 35 keywords.
Besides keywords, a programming language needs to define a set of operators, representing operations and actions.
For example, arithmetic operators (\eg, \texttt{+}, \texttt{-}, and \texttt{*}) and logical operators (\eg, \texttt{and}, \texttt{or}, and \texttt{not}) are two of most important categories.
In addition, a developer can use any string to name a variable, structure, function, class, etc., as long as this string is not conflicted with reserved keywords and operators, and follows the programming language specification.

When writing code, due to the program logic, the developer has limited flexibility to choose keywords and operators.
Only some keywords (such as \texttt{for} and \texttt{while}) and operators (such as \texttt{++}, \texttt{+1}) are exchangeable.
That is, the program logic is fixed when using a set of keywords and operators in a program.
In contrast, the name of a variable, function, or class has no impact on the program logic.

\lstset{style=mycstyle}
\begin{lstlisting}[language=C++,
emph={bubble_sort, begin, end, pred, it_end, finished, next, it},
label={code:goodname},caption={A piece of code with meaningful variable/function names.}, captionpos=b]{}
    template<typename It, typename Pred=std::less<typename std::iterator_traits<It>::value_type>>
    inline void bubble_sort(It begin, It end, Pred pred=Pred()){
        if ( std::distance( begin, end ) <= 1 ){ return; }
        auto it_end    = end;
        bool finished  = false;
        while ( !finished ){ //loop stop when no adjacent elements are not in required order. 
            finished = true;
            std::advance( it_end, -1 );
            // iteration over the whole sequence.
            for (auto it = begin; it! = it_end; ++ it ){
                auto next = detail::advance( it, 1 );
                // compare two adjacent elements and exchange them if not in required order.
                if (pred( * next, * it)){ 
                    std::swap( * it, * next);
                    finished = false;
                }
            }
        }   
    }
\end{lstlisting}


\begin{lstlisting}[language=C++,
emph={var1, var2, var3, var4, var5, var6, fun1, fun2},
label={code:badname},caption={The same code without meaningful variable/function names.}, captionpos=b]{}
    template<typename It, typename Fun2=std::less<typename std::iterator_traits<It>::value_type>>
    inline void fun1(It var1, It var2, Pred fun2=Fun2()){
        if ( std::distance( var1, var2 ) <= 1 ){ return; }
        auto var3  = var2;
        bool var4  = false;
        while ( !var4 ){
            var4 = true;
            std::advance( var3, -1 );
            for (auto var5 = var1; var5! = var3; ++ var5 ){
                auto var6 = detail::advance( var5, 1 );
                if (fun2( * var6, * var5)){
                    std::swap( * var5, * var6);
                    var4 = false;
                }
            }
        }   
    }
\end{lstlisting}

% \textcolor{red}{(Where is this bubble sorting function from? C++ standard library? Can we add some comments, i.e., programmer-readable annotation?)}
\autoref{code:goodname} and \autoref{code:badname} are two pieces of code with the same program logic~\textendash~\textit{bubble sorting}.
\autoref{code:goodname} is an implementation from the Web, which has well-named functions and variables whereas \autoref{code:badname} is anonymized by us. 
Through a quick glance, even a novice can easily conclude that \autoref{code:goodname} is a bubble-sort function based on the help from the literal meaning of the function name and the variable names.
However, it needs more time for an experienced analyst to go through this function line by line to understand the purpose of \autoref{code:badname}. 
Therefore, despite the exactly same program logic, \autoref{code:badname} is much more difficult to analyze.
In summary, although the name of a variable, function, or class has no impact on the program logic, it could also help the analyst to understand the purpose of a program if the literal meaning of the name aligns with the program logic.

From the above discussion, we give the definition of literal features and logical features:

\begin{definition}[Literal Features and Logical Features]
Given a piece of code, the \textbf{literal features} are features of the literal meaning of the variable names, function names and programmer-readable annotation. These feature could be removed without change the functionality of the code. The \textbf{logical features} are features that control the program logic. The keywords and operators defined by a programming language specification are logical features.
\end{definition}

Based on this definition, we can draw the following conclusions from the analysis of these two code snippets: 
1) a piece of code can be understood in two ways: \textit{literal analysis}, and \textit{logic analysis}.  2) The literal analysis makes a conclusion based on the names of variables, functions, etc., which is easier to analyze but is not always reliable. 3) The logic analysis requires a high-level understanding of the code, which is more reliable but hard to analyze.




==> sections/relatedworks.tex <==
\section{Related Works}
{\color{red}
In this section, we compare our attacking method with existing jailbreak attacks.
1. To by pass the safeguards, jailbreak prompts often utilize a combination of techniques. First, jailbreak prompts tend to be significantly longer, averaging 1.5× the length of regular prompts, with a mean token count of 555. 

}




